Regularized Federated Learning for Privacy-Preserving Dysarthric and Elderly Speech Recognition

Accurate recognition of dysarthric and elderly speech remains challenging to date. While privacy concerns have driven a shift from centralized approaches to federated learning (FL) to ensure data confidentiality, this further exacerbates the challenges of data scarcity, imbalanced data distribution and speaker heterogeneity. To this end, this paper conducts a systematic investigation of regularized FL techniques for privacy-preserving dysarthric and elderly speech recognition, addressing different levels of the FL process by 1) parameter-based, 2) embedding-based and 3) novel loss-based regularization. Experiments on the benchmark UASpeech dysarthric and DementiaBank Pitt elderly speech corpora suggest that regularized FL systems consistently outperform the baseline FedAvg system by statistically significant WER reductions of up to 0.55\% absolute (2.13\% relative). Further increasing communication frequency to one exchange per batch approaches centralized training performance.

==> bib_backup/new_bib_full_name.tex <==
@inproceedings{wang22k_interspeech,
  title     = {Conformer Based Elderly Speech Recognition System for Alzheimer’s Disease Detection},
  author    = {Tianzi Wang and Jiajun Deng and Mengzhe Geng and Zi Ye and Shoukang Hu and Yi Wang and Mingyu Cui and Zengrui Jin and Xunying Liu and Helen Meng},
  year      = {2022},
  booktitle = {Interspeech 2022},
  pages     = {4825--4829},
  doi       = {10.21437/Interspeech.2022-712},
  issn      = {2958-1796},
}

@INPROCEEDINGS{10095993,
  author={Wang, Yi and Deng, Jiajun and Wang, Tianzi and Zheng, Bo and Hu, Shoukang and Liu, Xunying and Meng, Helen},
  booktitle={ICASSP 2023 - 2023 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, 
  title={Exploiting Prompt Learning with Pre-Trained Language Models for Alzheimer’s Disease Detection}, 
  year={2023},
  volume={},
  number={},
  pages={1-5},
  keywords={Training;Costs;Bit error rate;Manuals;Signal processing;Linear programming;Alzheimer's disease;Prompt learning;AD detection;pre-trained language model},
  doi={10.1109/ICASSP49357.2023.10095993}}

@inproceedings{gulati20_interspeech,
  title     = {Conformer: Convolution-augmented Transformer for Speech Recognition},
  author    = {Anmol Gulati and James Qin and Chung-Cheng Chiu and Niki Parmar and Yu Zhang and Jiahui Yu and Wei Han and Shibo Wang and Zhengdong Zhang and Yonghui Wu and Ruoming Pang},
  year      = {2020},
  booktitle = {Interspeech 2020},
  pages     = {5036--5040},
  doi       = {10.21437/Interspeech.2020-3015},
  issn      = {2958-1796},
}

@ARTICLE{10584335,
  author={Hu, Shujie and Xie, Xurong and Geng, Mengzhe and Jin, Zengrui and Deng, Jiajun and Li, Guinan and Wang, Yi and Cui, Mingyu and Wang, Tianzi and Meng, Helen and Liu, Xunying},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing}, 
  title={Self-Supervised ASR Models and Features for Dysarthric and Elderly Speech Recognition}, 
  year={2024},
  volume={32},
  number={},
  pages={3561-3575},
  keywords={Speech recognition;Older adults;Data models;Task analysis;Decoding;Standards;Acoustics;Dysarthric Speech;Elderly Speech;Pre-trained ASR System;Wav2vec2.0;HuBERT;Multi-lingual XLSR},
  doi={10.1109/TASLP.2024.3422839}}


@article{ZVEROVA20193,
title = {Clinical aspects of Alzheimer's disease},
journal = {Clinical Biochemistry},
volume = {72},
pages = {3-6},
year = {2019},
author = {Martina Zvěřová}}

@article{AMMAR2020763,
title = {Language-related features for early detection of Alzheimer Disease},
journal = {Procedia Computer Science},
volume = {176},
pages = {763-770},
year = {2020},
doi = {https://doi.org/10.1016/j.procs.2020.09.071},
author = {Randa Ben Ammar and Yassine Ben Ayed}}

@INPROCEEDINGS{9413634,
  author={Ye, Zi and Hu, Shoukang and Li, Jinchao and Xie, Xurong and Geng, Mengzhe and Yu, Jianwei and Xu, Junhao and Xue, Boyang and Liu, Shansong and Liu, Xunying and Meng, Helen},
  booktitle={ICASSP 2021 - 2021 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, 
  title={Development of the Cuhk Elderly Speech Recognition System for Neurocognitive Disorder Detection Using the Dementiabank Corpus}, 
  year={2021},
  volume={},
  number={},
  pages={6433-6437},
  keywords={Training;Adaptation models;Perturbation methods;System performance;Senior citizens;Speech recognition;Transforms;Automatic Speech Recognition;Elderly Speech;Neurocognitive Disorder Detection;Dementia},
  doi={10.1109/ICASSP39728.2021.9413634}}



@InProceedings{pmlr-v54-mcmahan17a,
  title = 	 {{Communication-Efficient Learning of Deep Networks from Decentralized Data}},
  author = 	 {McMahan, Brendan and Moore, Eider and Ramage, Daniel and Hampson, Seth and Arcas, Blaise Aguera y},
  booktitle = 	 {Proceedings of the 20th International Conference on Artificial Intelligence and Statistics},
  pages = 	 {1273--1282},
  year = 	 {2017},
  editor = 	 {Singh, Aarti and Zhu, Jerry},
  volume = 	 {54},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {20--22 Apr},
  publisher =    {PMLR},
  pdf = 	 {http://proceedings.mlr.press/v54/mcmahan17a/mcmahan17a.pdf}
}

@inproceedings{MLSYS2020_1f5fe839,
 author = {Li, Tian and Sahu, Anit Kumar and Zaheer, Manzil and Sanjabi, Maziar and Talwalkar, Ameet and Smith, Virginia},
 booktitle = {Proceedings of Machine Learning and Systems},
 editor = {I. Dhillon and D. Papailiopoulos and V. Sze},
 pages = {429--450},
 title = {Federated Optimization in Heterogeneous Networks},
 volume = {2},
 year = {2020}
}


@article{shen2023federated,
  title={Federated mutual learning: a collaborative machine learning method for heterogeneous data, models, and objectives},
  author={Shen, Tao and Zhang, Jie and Jia, Xinkang and Zhang, Fengda and Lv, Zheqi and Kuang, Kun and Wu, Chao and Wu, Fei},
  journal={Frontiers of Information Technology \& Electronic Engineering},
  volume={24},
  number={10},
  pages={1390--1402},
  year={2023},
  publisher={Springer}
}

@article{huang2019patient,
  title={Patient clustering improves efficiency of federated machine learning to predict mortality and hospital stay time using distributed electronic medical records},
  author={Huang, Li and Shea, Andrew L and Qian, Huining and Masurkar, Aditya and Deng, Hao and Liu, Dianbo},
  journal={Journal of biomedical informatics},
  volume={99},
  pages={103291},
  year={2019},
  publisher={Elsevier}
}


@article{farahani2023towards,
  title={Towards A Personalized Clustered Federated Learning: A Speech Recognition Case Study},
  author={Farahani, Bahar and Tabibian, Shima and Ebrahimi, Hamid},
  journal={IEEE Internet of Things Journal},
  year={2023},
  publisher={IEEE}
}

@inproceedings{hsu2024cluster,
  title={A Cluster-based Personalized Federated Learning Strategy for End-to-End ASR of Dementia Patients},
  author={Hsu, Wei-Tung and Chen, Chin-Po and Lin, Yun-Shao and Lee, Chi-Chun},
  booktitle={Proc. Interspeech 2024},
  pages={2450--2454},
  year={2024}
}

@inproceedings{kim2008dysarthric,
  title={Dysarthric speech database for universal access research.},
  author={Kim, Heejin and Hasegawa-Johnson, Mark and Perlman, Adrienne and Gunderson, Jon R and Huang, Thomas S and Watkin, Kenneth L and Frame, Simone},
  booktitle={Interspeech},
  volume={2008},
  pages={1741--1744},
  year={2008}
}

@article{rudzicz2012torgo,
  title={The TORGO database of acoustic and articulatory speech from speakers with dysarthria},
  author={Rudzicz, Frank and Namasivayam, Aravind Kumar and Wolff, Talya},
  journal={Language resources and evaluation},
  volume={46},
  pages={523--541},
  year={2012},
  publisher={Springer}
}

@inproceedings{morris2004and,
  title={From WER and RIL to MER and WIL: improved evaluation measures for connected speech recognition.},
  author={Morris, Andrew Cameron and Maier, Viktoria and Green, Phil D},
  booktitle={Interspeech},
  pages={2765--2768},
  year={2004}
}

@article{hsu2021hubert,
  title={Hubert: Self-supervised speech representation learning by masked prediction of hidden units},
  author={Hsu, Wei-Ning and Bolte, Benjamin and Tsai, Yao-Hung Hubert and Lakhotia, Kushal and Salakhutdinov, Ruslan and Mohamed, Abdelrahman},
  journal={IEEE/ACM transactions on audio, speech, and language processing},
  volume={29},
  pages={3451--3460},
  year={2021},
  publisher={IEEE}
}

@inproceedings{bisani2004bootstrap,
  title={Bootstrap estimates for confidence intervals in ASR performance evaluation},
  author={Bisani, Maximilian and Ney, Hermann},
  booktitle={2004 IEEE International Conference on Acoustics, Speech, and Signal Processing},
  volume={1},
  pages={I--409},
  year={2004},
  organization={IEEE}
}


@article{becker1994natural,
  title={The natural history of Alzheimer's disease: description of study cohort and accuracy of diagnosis},
  author={Becker, James T and Boiler, Fran{\c{c}}ois and Lopez, Oscar L and Saxton, Judith and McGonigle, Karen L},
  journal={Archives of neurology},
  volume={51},
  number={6},
  pages={585--594},
  year={1994},
  publisher={American Medical Association}
}

@article{liu2021recent,
  title={{Recent Progress in the CUHK Dysarthric Speech Recognition System}},
  author={Liu, Shansong and others},
  volume={29},
  pages={2267--2281},
  journal={TASLP},
  year={2021},
  publisher={IEEE}
}

@article{smith1987temporal,
  title={{Temporal characteristics of the speech of normal elderly adults}},
  journal={JSLHR},
  year={1987},
  author={Smith, Bruce L and others},
  volume={30},
  pages={522--529},
  publisher={ASHA}
}

@article{kodrasi2020spectro,
  title={{Spectro-temporal sparsity characterization for dysarthric speech detection}},
  journal={TASLP},
  publisher={IEEE},
  author={Kodrasi, Ina and Bourlard, Herv{\'e}},
  volume={28},
  pages={1210--1222},
  year={2020},
}

@inproceedings{hard2020training,
  author    = {Hard, A. and Partridge, K. and Nguyen, C. and Subrahmanya, N. and Shah, A. and Zhu, P. and Moreno, I. L. and Mathews, R.},
  title     = {Training Keyword Spotting Models on Non-IID Data with Federated Learning},
  booktitle = {Proc. Interspeech 2020},
  pages     = {4343--4347},
  year      = {2020},
  doi       = {10.21437/Interspeech.2020-3023}
}


@inproceedings{leroy2019federated,
  title={Federated learning for keyword spotting},
  author={Leroy, David and Coucke, Alice and Lavril, Thibaut and Gisselbrecht, Thibault and Dureau, Joseph},
  booktitle={ICASSP 2019-2019 IEEE international conference on acoustics, speech and signal processing (ICASSP)},
  pages={6341--6345},
  year={2019},
  organization={IEEE}
}

@inproceedings{dimitriadis2020federated,
  title={A Federated Approach in Training Acoustic Models.},
  author={Dimitriadis, Dimitrios and Ken'ichi Kumatani, Robert Gmyr and Gmyr, Robert and Gaur, Yashesh and Eskimez, Sefik Emre},
  booktitle={Interspeech},
  pages={981--985},
  year={2020}
}

@inproceedings{Granqvist2020,
  author = {Filip Granqvist and Matt Seigel and Rogier van Dalen and Áine Cahill and Stephen Shum and Matthias Paulik},
  title = {Improving On-Device Speaker Verification Using Federated Learning With Privacy},
  booktitle = {INTERSPEECH},
  year = {2020}
}

@inproceedings{cui2021federated,
  title={Federated acoustic modeling for automatic speech recognition},
  author={Cui, Xiaodong and Lu, Songtao and Kingsbury, Brian},
  booktitle={ICASSP 2021-2021 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={6748--6752},
  year={2021},
  organization={IEEE}
}

@inproceedings{latif2020federated,
  title={Federated learning for speech emotion recognition applications},
  author={Latif, Siddique and Khalifa, Sara and Rana, Rajib and Jurdak, Raja},
  booktitle={2020 19th ACM/IEEE International Conference on Information Processing in Sensor Networks (IPSN)},
  pages={341--342},
  year={2020},
  organization={IEEE}
}

@inproceedings{tsouvalas2022privacy,
  title={Privacy-preserving speech emotion recognition through semi-supervised federated learning},
  author={Tsouvalas, Vasileios and Ozcelebi, Tanir and Meratnia, Nirvana},
  booktitle={2022 IEEE International Conference on Pervasive Computing and Communications Workshops and other Affiliated Events (PerCom Workshops)},
  pages={359--364},
  year={2022},
  organization={IEEE}
}

@inproceedings{feng2022semi,
  title={{Semi-fedSER: Semi-supervised learning for speech emotion recognition on federated learning using multiview pseudo-labeling},
  author={Feng, Tiantian and Narayanan, Shrikanth}},
  booktitle={INTERSPEECH},
  year={2022}
}

@inproceedings{zhang2024stealthy,
  title={Stealthy backdoor attack towards federated automatic speaker verification},
  author={Zhang, Longling and Liu, Lyqi and Meng, Dan and Wang, Jun and Hu, Shengshan},
  booktitle={ICASSP 2024-2024 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={1311--1315},
  year={2024},
  organization={IEEE}
}

@article{chen2023learning,
  title={Learning domain-heterogeneous speaker recognition systems with personalized continual federated learning},
  author={Chen, Zhiyong and Xu, Shugong},
  journal={EURASIP Journal on Audio, Speech, and Music Processing},
  volume={2023},
  number={1},
  pages={33},
  year={2023},
  publisher={Springer}
}

@inproceedings{gao2022end,
  title={End-to-end speech recognition from federated acoustic models},
  author={Gao, Yan and Parcollet, Titouan and Zaiem, Salah and Fernandez-Marques, Javier and de Gusmao, Pedro PB and Beutel, Daniel J and Lane, Nicholas D},
  booktitle={ICASSP 2022-2022 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={7227--7231},
  year={2022},
  organization={IEEE}
}

@inproceedings{azam2023importance,
  title={Importance of smoothness induced by optimizers in fl4asr: Towards understanding federated learning for end-to-end asr},
  author={Azam, Sheikh Shams and Likhomanenko, Tatiana and Pelikan, Martin and others},
  booktitle={2023 IEEE Automatic Speech Recognition and Understanding Workshop (ASRU)},
  pages={1--8},
  year={2023},
  organization={IEEE}
}

@inproceedings{guliani2021training,
  title={Training speech recognition models with federated learning: A quality/cost framework},
  author={Guliani, Dhruv and Beaufays, Fran{\c{c}}oise and Motta, Giovanni},
  booktitle={ICASSP 2021-2021 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={3080--3084},
  year={2021},
  organization={IEEE}
}

@article{kan2024parameter,
  title={Parameter-Efficient Transfer Learning under Federated Learning for Automatic Speech Recognition},
  author={Kan, Xuan and Xiao, Yonghui and Yang, Tien-Ju and Chen, Nanxin and Mathews, Rajiv},
  journal={arXiv preprint arXiv:2408.11873},
  year={2024}
}

@inproceedings{yu2021federated,
  title={{Federated learning in ASR: Not as easy as you think}},
  author={Yu, Wentao and Freiwald, Jan and Tewes, S{\"o}ren and Huennemeyer, Fabien and Kolossa, Dorothea},
  booktitle={Speech Communication; 14th ITG Conference},
  pages={1--5},
  year={2021},
  organization={VDE}
}

@inproceedings{azam2023federated,
  title={Federated Learning for Speech Recognition: Revisiting Current Trends Towards Large-Scale ASR},
  author={Azam, Sheikh Shams and Pelikan, Martin and Feldman, Vitaly and Talwar, Kunal and Silovsky, Jan and Likhomanenko, Tatiana},
  booktitle={International Workshop on Federated Learning in the Age of Foundation Models in Conjunction with NeurIPS 2023},
  year={2023}
}

@article{pelikan2023federated,
  title={Federated learning with differential privacy for end-to-end speech recognition},
  author={Pelikan, Martin and Azam, Sheikh Shams and Feldman, Vitaly and Silovsky, Jan and Talwar, Kunal and Likhomanenko, Tatiana and others},
  journal={arXiv preprint arXiv:2310.00098},
  year={2023}
}

@inproceedings{nandury2021cross,
  title={Cross-silo federated training in the cloud with diversity scaling and semi-supervised learning},
  author={Nandury, Kishore and Mohan, Anand and Weber, Frederick},
  booktitle={ICASSP 2021-2021 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={3085--3089},
  year={2021},
  organization={IEEE}
}


@inproceedings{meerza2022fair,
  title={Fair and Privacy-Preserving Alzheimer's Disease Diagnosis Based on Spontaneous Speech Analysis via Federated Learning},
  author={Meerza, Syed Irfan Ali and Li, Zhuohang and Liu, Luyang and Zhang, Jiaxin and Liu, Jian},
  booktitle={2022 44th Annual International Conference of the IEEE Engineering in Medicine \& Biology Society (EMBC)},
  pages={1362--1365},
  year={2022},
  organization={IEEE}
}

@inproceedings{arasteh2023federated,
  title={Federated learning for secure development of AI models for Parkinson's disease detection using speech from different languages},
  author={Arasteh, Soroosh Tayebi and Rios-Urrego, Cristian David and Noeth, Elmar and Maier, Andreas and Yang, Seung Hee and Rusz, Jan and Orozco-Arroyave, Juan Rafael},
  booktitle={INTERSPEECH},
  year={2023}
}

@inproceedings{kalabakov2024comparative,
  title={A Comparative Analysis of Federated Learning for Speech-Based Cognitive Decline Detection},
  author={Kalabakov, Stefan and Gonzalez-Machorro, Monica and Eyben, Florian and Schuller, Bj{\"o}rn W and Arnrich, Bert},
  booktitle={Proc. Interspeech 2024},
  pages={2455--2459},
  year={2024}
}

@ARTICLE{GreidiCohen2024,
  author = {Ran Greidi and Kobi Cohen},
  title = {Sparse Training for Federated Learning With Regularized Error Correction},
  journal = {IEEE Journal of Selected Topics in Signal Processing},
  year = {2024},
  volume = {18},
  number = {6},
  doi = {10.1109/JSTSP.2024.10684110}
}

@INPROCEEDINGS{Tun2023,
  author = {Ye Lin Tun and Chu Myaet Thwal and Yu Min Park and Seong-Bae Park and Choong Seon Hong},
  title = {Federated Learning with Intermediate Representation Regularization},
  booktitle = {Proceedings of the 2023 IEEE International Conference on Big Data (BigComp)},
  year = {2023},
  doi = {10.1109/BigComp.2023.757800A056},}
}

@article{kullback1951information,
  title={On information and sufficiency},
  author={Kullback, Solomon and Leibler, Richard A},
  journal={The annals of mathematical statistics},
  volume={22},
  number={1},
  pages={79--86},
  year={1951},
  publisher={JSTOR}
}

@inproceedings{dong2018speech,
  title={Speech-transformer: a no-recurrence sequence-to-sequence model for speech recognition},
  author={Dong, Linhao and Xu, Shuang and Xu, Bo},
  booktitle={2018 IEEE international conference on acoustics, speech and signal processing (ICASSP)},
  pages={5884--5888},
  year={2018},
  organization={IEEE}
}

@article{geng2022speaker,
  title={Speaker adaptation using spectro-temporal deep features for dysarthric and elderly speech recognition},
  author={Geng, Mengzhe and Xie, Xurong and Ye, Zi and Wang, Tianzi and Li, Guinan and Hu, Shujie and Liu, Xunying and Meng, Helen},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing},
  volume={30},
  pages={2597--2611},
  year={2022},
  publisher={IEEE}
}

@inproceedings{baskar2022speaker,
  title={{Speaker adaptation for Wav2vec2 based dysarthric ASR}},
  author={Baskar, Murali Karthick and Herzig, Tim and Nguyen, Diana and Diez, Mireia and Polzehl, Tim and Burget, Luk{\'a}{\v{s}} and {\v{C}}ernock{\`y}, Jan},
  booktitle={INTERPSEECH},
  year={2022}
}

@inproceedings{wang2024enhancing,
  title={Enhancing Pre-trained ASR System Fine-tuning for Dysarthric Speech Recognition using Adversarial Data Augmentation},
  author={Wang, Huimeng and Jin, Zengrui and Geng, Mengzhe and Hu, Shujie and Li, Guinan and Wang, Tianzi and Xu, Haoning and Liu, Xunying},
  booktitle={ICASSP 2024-2024 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={12311--12315},
  year={2024},
  organization={IEEE}
}

@article{jin2023personalized,
  title={Personalized adversarial data augmentation for dysarthric and elderly speech recognition},
  author={Jin, Zengrui and Geng, Mengzhe and Deng, Jiajun and Wang, Tianzi and Hu, Shujie and Li, Guinan and Liu, Xunying},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing},
  year={2023},
  publisher={IEEE}
}

@article{wang2025phone,
  title={Phone-purity Guided Discrete Tokens for Dysarthric Speech Recognition},
  author={Wang, Huimeng and Xie, Xurong and Geng, Mengzhe and Hu, Shujie and Xu, Haoning and Chen, Youjun and Li, Zhaoqing and Deng, Jiajun and Liu, Xunying},
  journal={arXiv preprint arXiv:2501.04379},
  year={2025}
}

@inproceedings{ye2021development,
  title={Development of the cuhk elderly speech recognition system for neurocognitive disorder detection using the dementiabank corpus},
  author={Ye, Zi and Hu, Shoukang and Li, Jinchao and Xie, Xurong and Geng, Mengzhe and Yu, Jianwei and Xu, Junhao and Xue, Boyang and Liu, Shansong and Liu, Xunying and others},
  booktitle={ICASSP 2021-2021 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={6433--6437},
  year={2021},
  organization={IEEE}
}

@article{yue2022acoustic,
  title={Acoustic modelling from raw source and filter components for dysarthric speech recognition},
  author={Yue, Zhengjun and Loweimi, Erfan and Christensen, Heidi and Barker, Jon and Cvetkovic, Zoran},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing},
  volume={30},
  pages={2968--2980},
  year={2022},
  publisher={IEEE}
}

@article{williamson2024balancing,
  title={Balancing privacy and progress: a review of privacy challenges, systemic oversight, and patient perceptions in AI-driven healthcare},
  author={Williamson, Steven M and Prybutok, Victor},
  journal={Applied Sciences},
  volume={14},
  number={2},
  pages={675},
  year={2024},
  publisher={MDPI}
}

@article{verbraeken2020survey,
  title={A survey on distributed machine learning},
  author={Verbraeken, Joost and Wolting, Matthijs and Katzy, Jonathan and Kloppenburg, Jeroen and Verbelen, Tim and Rellermeyer, Jan S},
  journal={Acm computing surveys (csur)},
  volume={53},
  number={2},
  pages={1--33},
  year={2020},
  publisher={ACM New York, NY, USA}
}

@inproceedings{du2024communication,
  title={Communication-Efficient Personalized Federated Learning for Speech-to-Text Tasks},
  author={Du, Yichao and Zhang, Zhirui and Yue, Linan and Huang, Xu and Zhang, Yuqing and Xu, Tong and Xu, Linli and Chen, Enhong},
  booktitle={ICASSP 2024-2024 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={10001--10005},
  year={2024},
  organization={IEEE}
}
